Hydrogen in Practice: A Global Review of Demonstration Projects from Production to Integration

Hydrogen technology has the potential to address various challenges related to integrating low- and zero-carbon energy sources, as well as achieving carbon neutrality. It provides valuable solutions for transitioning to net-zero emission energy systems on a global scale. The implementation of hydrogen production and integration demonstration projects has received significant attention around the world and strong support from governments, highlighting the crucial role of such initiatives in the advancement of hydrogen energy. However, research in this area remains limited, particularly in terms of comprehensive and systematic reviews of industrial practices under real-world conditions. To bridge this gap, this article provides an in-depth review of hydrogen production, storage, and industrial applications, summarizing key features of thirteen exemplary hydrogen demonstration projects from around the world. The goal is to offer insights and guidance for the large-scale deployment of hydrogen energy while identifying potential technological pathways for the future.

==> PRJ.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[font=\small,>=stealth,x=1cm,y=1cm]
%----- Colors
\definecolor{blueH}{HTML}{3B82F6}   % Blue hydrogen
\definecolor{greenH}{HTML}{10B981}  % Green hydrogen
\definecolor{neutral}{gray}{0.25}
\definecolor{coTwo}{HTML}{EF4444}   % CO2 arrows
%----- Layout
\def\W{3.2}   % column width
\def\H{1.4}   % row height
\def\N{5}     % number of rows
% Column titles
\node[anchor=west] at (0, \N*\H+0.5) {\bf Project overview (Production $\rightarrow$ Storage/Distribution $\rightarrow$ Use)};
\foreach \i/\txt in {0/Feedstock,1/Hydrogen Production,2/Storage \& Distribution,3/End Use / Grid Service}{
  \node[align=center] at (\i*\W+0.5*\W, \N*\H) {\bf \txt};
}
\node[align=center] at (4*\W+0.65, \N*\H) {\bf KPIs (LHV)};
% Row labels
\foreach \r/\name in {4/HyNet,3/H2Teesside,2/H2FUTURE,1/Demo4Grid,0/H2 Green Steel}{
  \node[anchor=east] at (-0.15, \r*\H+0.7*\H) {\bf \name};
}

%----- Helper to draw a row: \row{y}{feed}{prod}{store}{use}{kpi}{color}
\newcommand{\row}[6]{
  % Boxes
  \foreach \c in {0,1,2,3}{
    \draw[rounded corners=2pt] (\c*\W, #1) rectangle (\c*\W+\W, #1+\H);
  }
  % Text in boxes
  \node[align=center,text=neutral] at (0*\W+0.5*\W, #1+0.5*\H) {#2};
  \node[align=center,text=#6,very thick] at (1*\W+0.5*\W, #1+0.5*\H) {#3};
  \node[align=center,text=neutral] at (2*\W+0.5*\W, #1+0.5*\H) {#4};
  \node[align=center,text=neutral] at (3*\W+0.5*\W, #1+0.5*\H) {#5};
  % Arrows
  \draw[->,thick] (0*\W+\W, #1+0.5*\H) -- (1*\W, #1+0.5*\H);
  \draw[->,thick] (1*\W+\W, #1+0.5*\H) -- (2*\W, #1+0.5*\H);
  \draw[->,thick] (2*\W+\W, #1+0.5*\H) -- (3*\W, #1+0.5*\H);
  % KPI bar
  \draw[rounded corners=2pt] (4*\W, #1) rectangle (4*\W+2.8, #1+\H);
  \node[align=left] at (4*\W+0.15, #1+\H-0.28) {\scriptsize #6};
  \node[align=left] at (4*\W+0.15, #1+\H-0.62) {\scriptsize #7};
  \node[align=left] at (4*\W+0.15, #1+\H-0.96) {\scriptsize #8};
}

%----- Rows (content)
% HyNet (blue H2)
\row{4*\H}{Natural gas}{Auto-thermal Reforming (ATR)}{Pipe network \& tube trailers}{Refueling \& Gas turbines}{blueH}
% KPI text for HyNet
\node[anchor=west] at (4*\W+0.15,4*\H+0.96) {\scriptsize \textbf{H$_2$ cap.}: 890 MW $\approx$ 641 t/d; peak 380 MW $\approx$ 274 t/d};
\node[anchor=west] at (4*\W+0.15,4*\H+0.62) {\scriptsize \textbf{CCS}: $\sim$93\% to Liverpool Bay storage};
\node[anchor=west] at (4*\W+0.15,4*\H+0.28) {\scriptsize \textbf{Note}: 15--20\% H$_2$ blend to CCGT};

% CO2 arrow (HyNet)
\draw[->,coTwo,very thick,dashed] (1*\W+0.2,4*\H+0.15) .. controls (1.2*\W,4.65*\H) .. (2.0*\W-0.2,4.95*\H)
node[pos=0.55,above,coTwo] {\scriptsize CO$_2$ to storage};

% H2Teesside (blue H2)
\row{3*\H}{Natural gas}{Steam Methane Reforming (SMR)}{Pipeline \& tube truck}{Industrial end-users}{blueH}
\node[anchor=west] at (4*\W+0.15,3*\H+0.96) {\scriptsize \textbf{H$_2$ cap.}: —};
\node[anchor=west] at (4*\W+0.15,3*\H+0.62) {\scriptsize \textbf{CCS}: Capture $\rightarrow$ Endurance saline aquifer};
\node[anchor=west] at (4*\W+0.15,3*\H+0.28) {\scriptsize \textbf{Tech}: OASE absorption; LCH route};

\draw[->,coTwo,very thick,dashed] (1*\W+0.2,3*\H+0.15) .. controls (1.2*\W,3.65*\H) .. (2.0*\W-0.2,3.95*\H);

% H2FUTURE (green H2)
\row{2*\H}{Wind/solar/hydro}{PEM Electrolyzer}{Compressed H$_2$ storage}{Refineries / Fertilizer / Steel}{greenH}
\node[anchor=west] at (4*\W+0.15,2*\H+0.96) {\scriptsize \textbf{H$_2$ cap.}: 20,000 Nm$^3$/h $\approx$ 60 MW $\approx$ 43 t/d};
\node[anchor=west] at (4*\W+0.15,2*\H+0.62) {\scriptsize \textbf{Stack}: 1 A/cm$^2$, 150 bar, $\eta \sim$80\%};
\node[anchor=west] at (4*\W+0.15,2*\H+0.28) {\scriptsize \textbf{Note}: public demos also report 6 MW units};

% Demo4Grid (green H2 + grid)
\row{1*\H}{Renewables}{Electrolyzer}{H$_2$ buffer storage}{Grid service (FCR/FRR)}{greenH}
\node[anchor=west] at (4*\W+0.15,1*\H+0.96) {\scriptsize \textbf{Role}: Flexible load for frequency control};
\node[anchor=west] at (4*\W+0.15,1*\H+0.62) {\scriptsize \textbf{Signals}: seconds--minutes response};
\node[anchor=west] at (4*\W+0.15,1*\H+0.28) {\scriptsize \textbf{Value}: curtailment reduction + ancillary services};

% H2 Green Steel (green H2 for DRI)
\row{0*\H}{Water + renewables}{Electrolysis}{On-site storage}{DRI $\rightarrow$ EAF steel}{greenH}
\node[anchor=west] at (4*\W+0.15,0*\H+0.96) {\scriptsize \textbf{Use}: Continuous H$_2$ for DRI; offgas H$_2$O};
\node[anchor=west] at (4*\W+0.15,0*\H+0.62) {\scriptsize \textbf{Need}: long-hour stable supply and power};
\node[anchor=west] at (4*\W+0.15,0*\H+0.28) {\scriptsize \textbf{Scale}: —};

% Legend
\draw[rounded corners=2pt] (-0.2,-0.9) rectangle (6*\W+0.7,-0.3);
\node[anchor=west] at (0.0,-0.6) {\scriptsize \textbf{Legend:} \textcolor{blueH}{Blue} = NG+CCS; \textcolor{greenH}{Green} = Renewable+Electrolysis; 
\textcolor{coTwo}{\dashuline{Red dashed}} = CO$_2$ to storage. LHV=33.33 kWh/kg; 1 Nm$^3$=0.0899 kg $\approx$ 3.0 kWh.}
\end{tikzpicture}
\caption{Unified overview of five hydrogen demonstration projects. All capacities shown on LHV basis.}
\end{figure}

